Position: Leverage Foundational Models for Black-Box Optimization

Undeniably, Large Language Models (LLMs) have stirred an extraordinary wave of innovation in the machine learning research domain, resulting in substantial impact across diverse fields such as reinforcement learning, robotics, and computer vision. Their incorporation has been rapid and transformative, marking a significant paradigm shift in the field of machine learning research. However, the field of experimental design, grounded on black-box optimization, has been much less affected by such a paradigm shift, even though integrating LLMs with optimization presents a unique landscape ripe for exploration. In this position paper, we frame the field of black-box optimization around sequence-based foundation models and organize their relationship with previous literature. We discuss the most promising ways foundational language models can revolutionize optimization, which include harnessing the vast wealth of information encapsulated in free-form text to enrich task comprehension, utilizing highly flexible sequence models such as Transformers to engineer superior optimization strategies, and enhancing performance prediction over previously unseen search spaces.

==> introduction.tex <==
The ability to intelligently suggest new promising designs and experimentally validate such designs has been the key to an overwhelming number of applications, ranging from \cite{} to \cite{}. Central to experimental design is efficiently attempting new configurations given previous attempts and feedbacks. Framed as a mathematical problem, the optimization community has commonly referred to the study of such abilities as \textit{blackbox optimization}. The term "blackbox" refers to having minimal assumptions on the outcome, or \textit{objective}, to be optimized, either intentionally to simplify the problem setting, or due to inherent lack of information about the objective.

\textcolor{red}{Picture of example problems}

A fundamental quest in the field of blackbox optimization is finding more intelligent methods to efficiently propose promising suggestions which lead to better objectives. Yet ironically, it is precisely the blackbox assumption which must be broken to achieve better methods. Hand-designed algorithms inherently assume a mathematical prior (e.g. smoothness) or inductive bias on the problem, and the most performant methods are usually those which in fact, exploit the problem information as much as possible. 

The emergence of deep learning has resulted in the learnability of these inductive biases using neural networks trained from data, and further automated the end-to-end act of proposing promising new suggestions. A key question is: \textit{How far can we take learned optimization?} Ideally, a learned optimizer over any domain should have the following key capabilities:

\begin{itemize}
\itemsep0em 
\item Integrate previous evaluations into its decision making.
\item Perform exploration to gather novel information and exploitation to refine promising suggestions. 
\item Make valid suggestions over constraints from a given search space.
\item Condition behavior according to problem scenario and user commands.
\end{itemize}

So far, recent advances in sequence modelling \cite{} have made some of these behaviors possible. The core Transformer architecture \cite{} can utilize previous evaluations via its in-context learning properties, and can perform a variety of algorithmic tasks due to its strong expressiveness. Furthermore, by expressing text as token sequences, language models have facilitated expressing problem information in a free-form manner, thereby making optimization applicable to a variety of search spaces in new domains unapplicable previously. 

Despite these significantly new upgrades, certain ideal behaviors have still not emerged fully. 

%A wider vision however, ...  Such behaviors are still not emergent, and thus more research needs to be done 
%Here is the outline of the paper.
%and ultimately in multimodal foundation models allow us to support more flexible forms of input space and incorpoate diverse user specifications

\textcolor{red}{Exemplified with a ChatGPT example/illustration of language-based BBO.}




==> temp.tex <==
\begin{table*}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{|c|c|c|c|c|c|c|}\hline
%\backslashbox{Application}{Method}

Applications / Method & Non-learnable & Feature-based & Sequence-Based & Attention-Based & Token-Based & LLM-based \\
\hline
Flat Primitives & Hill-Climb & Bayesian Optimization & \cite{chen2017learning} & XX & \cite{chen2022towards} & \cite{yang2023large} \\
\hline
Conditional + Dynamic & Mutation-based & Combinatorial GPs &  \cite{rl_co} & XX  & & \\
\hline
Genetic Programming & Mutation-Based & ?? & ?? & ?? & ?? & ??\\
\hline
Unrestricted Code & N/A & N/A & N/A & N/A & N/A & FunSearch \\
\hline
Prompts & N/A & N/A & N/A & N/A & N/A & Prompt-Breeder \\
\hline


\end{tabular}
}
\caption{}
\end{table*}





\begin{table*}[t]
\centering
\begin{tabular}{ |p{3.2cm}|p{3cm} |p{1.75cm}|p{2.25cm}|p{4cm}|  }
\hline
\multicolumn{5}{|c|}{Related Work Comparison} \\
\hline
Reference & Surrogate Model & Attention & Token Model & Applications \\
\hline
\citet{rl_co} & RNN & \xmark & \xmark & BBO \\
\citet{chen2017learning} & RNN   & \xmark & \xmark & BBO, HPO\\
\citet{lange2023discovering} & ES &  \cmark & \xmark & BBO, Neuroevolution\\
\citet{lange2023discovering2} & GA & \cmark & \xmark & BBO, Neuroevolution, HPO\\
\citet{chen2022towards} & T5 Transformer & \cmark & \cmark & BBO, HPO\\
\citet{lehman2023evolution} & LLM & \cmark & \cmark & Code\\
\citet{chen2023evoprompting} & LLM & \cmark & \cmark & Code, NAS\\
\citet{meyerson2023language} & LLM & \cmark & \cmark & Prompts, Code, Text\\
\citet{yang2023large} & LLM & \cmark & \cmark & Regression, Prompts\\
\citet{zhang2023using} & LLM & \cmark & \cmark & BBO, HPO\\
\hline
\end{tabular}
\caption{Related work overview comparison.}
\end{table*}


